Clique-Based Separators for Geometric Intersection Graphs

Let $F$ be a set of $n$ objects in the plane and let $G(F)$ be its intersection graph. A balanced clique-based separator of $G(F)$ is a set $S$ consisting of cliques whose removal partitions $G(F)$ into components of size at most $\delta n$, for some fixed constant $\delta<1$. The weight of a clique-based separator is defined as $\sum_{C\in S}\log (|C|+1)$. Recently De Berg et al. (SICOMP 2020) proved that if $S$ consists of convex fat objects, then $G(F)$ admits a balanced clique-based separator of weight $O(\sqrt{n})$. We extend this result in several directions, obtaining the following results. Map graphs admit a balanced clique-based separator of weight $O(\sqrt{n})$, which is tight in the worst case. Intersection graphs of pseudo-disks admit a balanced clique-based separator of weight $O(n^{2/3}\log n)$. If the pseudo-disks are polygonal and of total complexity $O(n)$ then the weight of the separator improves to $O(\sqrt{n}\log n)$. Intersection graphs of geodesic disks inside a simple polygon admit a balanced clique-based separator of weight $O(n^{2/3}\log n)$. Visibility-restricted unit-disk graphs in a polygonal domain with $r$ reflex vertices admit a balanced clique-based separator of weight $O(\sqrt{n}+r\log(n/r))$, which is tight in the worst case. These results immediately imply sub-exponential algorithms for MAXIMUM INDEPENDENT SET (and, hence, VERTEX COVER), for FEEDBACK VERTEX SET, and for $q$-COLORING for constant $q$ in these graph classes.

==> OLD/old-map-graphs.tex <==
%--------------------------------------------------------------------------------------
\section{Map graphs}
\label{sec:map-graphs}
%--------------------------------------------------------------------------------------
Let $S$ be a set of $n$ interior-disjoint objects in the plane.
We say that two objects from~$S$ are \emph{neighbors} if $\bd o_i\cap \bd o_j \neq \emptyset$.
We say that two neighbors $o_i$ and $o_j$ are \emph{proper neighbors} if $\bd o_i\cap \bd o_j$
has non-zero length; otherwise they are \emph{improper neighbors}.
Recall that the intersection graph $\ig(S)$ has an edge between two objects if and only
if they are neighbors. We define the \emph{proper intersection graph} of $S$,
denoted by $\gpr(S)$, to be the graph with node set $S$ where we only add edges
between proper neighbors. Since proper intersection graphs are planar, they are
more convenient to work with. Hence, we first describe a procedure that constructs,
given a set $S$, a set $S^*\cup C$ such that $\gpr(S^*\cup C)$ is a suitable representation of
$\ig(S)$.
\medskip

%--------------------------------------------------------------------------------------
\mypara{Regularizing map graphs.}
%--------------------------------------------------------------------------------------
Let~$\subdiv(S)$ be the subdivision defined by~$S$.
Because we do not require the objects to have constant complexity, any two object 
boundaries can meet arbitrarily many times. As a result the number of vertices, 
edges and faces of~$\subdiv(S)$ need not be linear in~$n$. To avoid this, we 
first modify the objects from $S$, as follows. 

Let $H$ be the set of bounded faces of $\subdiv(S)$ whose boundary consists of 
boundary pieces of exactly two objects in~$S$. We add each face $f\in H$
arbitrarily to one of two objects contributing to its boundary.
Let $S^+$ be the resulting set of objects. Note that each object~in~$S$ is contained
in exactly one object in~$S^+$. Moreover, two objects $o_i,o_j\in S$ are neighbors
if and only if the corresponding objects in~$o^+_i,o_j^+\in S^+$ are neighbors:
proper neighbors stay proper neighbors, improper neighbors either stay improper
neighbors or become proper neighbors, and no new neighbors are introduced.

Now consider the subdivision~$\subdiv(S^+)$. Observe that $\subdiv(S^+)$ has a 
linear number of faces and, hence, a linear number of edges and vertices. 
    \mdb{Add argument}  
We say that a vertex~$v$ of $\subdiv(S^+)$ is \emph{irregular}
if there are at least two objects $o_i,o_j$ that touch at~$v$, meaning that in 
a sufficiently small neighborhood of~$v$ we have $\bd o_i \cap \bd o_j = v$;
see Fig.~\ref{fi:regularize} for an illustration. A vertex that is not
irregular is called \emph{regular}.
Let $\Vir$ be the set of non-regular vertices~of~$\subdiv(S^+)$. 
For an irregular vertex~$v$, let $S_v\subseteq S$ be the set of objects
whose boundary contains~$v$. For each irregular vertex~$v$, we place a small 
disk $b_v$ with its center at~$v$. The disks $b_v$ are chosen
small enough so that each disk~$b_v$ intersects only the objects in $S_v$;
it does not intersect any  no other objects from~$S$ nor any other disk~$b_{v'}$.
We call $b_v$ a \emph{connector}. Let $C := \{ b_v : v\in \Vir \}$
be the set of all connectors.
%--------------------------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics{Figures/regularize.pdf}
\end{center}
\caption{(i) A set $S$ of interior-disjoint objects, with non-regular vertices are shown in red.
           (ii) The regularization of $\ig(S)$ is shown in blue.
                The dark grey disks with a red boundary are the connectors.}
\label{fi:regularize}
\end{figure}
%--------------------------------------------------------------------------------------
For each object $o^+_i\in S^+$, we now define $o^*_i := o_i^+ \setminus \bigcup_{v\in \Vir} b_v$. 
Thus $o^*_i$ is obtained from~$o_i^+$ by removing the parts of $o_i^+$ inside the connectors
of its incident irregular vertices. Let $S^*$ be the resulting set of objects.
We summarize the important properties of the set~$S^*\cup C$.
\begin{itemize}
\item The total number of objects and disks in $S^*\cup C$ is $O(n)$.
\item Each object $o_i\in S$ corresponds to exactly one object in~$o^*_i\in S^*$.
\item If two objects $o_i,o_j\in S$ are proper neighbors then the corresponding
      objects $o^*_i,o^*_j\in S^*$ are proper neighbors.
\item If two objects $o_i,o_j\in S$ are improper neighbors then $o^*_i$
      and $o^*_j$ are proper neighbors or there is a connector
      $b_v\in C$ that is a proper neighbor of both~$o^*_i$ and $o^*_j$.
\item If $o^*_i,o^*_j\in S$ are neighbors, or $o^*_i$ and $o^*_j$
      have a connector $b_v$ as common neighbor, then $o_i,o_j$ are neighbors.
\end{itemize}
We call $\gpr(S^*\cup C)$ the \emph{regularization} of~$\ig(S)$. 
Using $\gpr(S^*\cup C)$ we can now easily prove the following separator theorem for map graphs. 

%--------------------------------------------------------------------------------------
\begin{theorem}\label{th:map-graph-separator}
Let $S$ be a set of $n$ interior-disjoint regions in the plane. Then the 
intersection graph $\ig(S)$ has a clique-based separator of weight~$O(\sqrt{n})$.
\end{theorem}
%--------------------------------------------------------------------------------------
\begin{proof}
Let $\gpr(S^*\cup C)$ be the regularization
of $\ig(S)$. We turn $\gpr(S^*\cup C)$ into a vertex-weighted graph by
setting $\weight(o^*_i) := 1$ for each object in $S^*$, and setting
\[
\weight(b_v) := \mbox{ number of neighbors of~$b_v$}
\]
for each $b_v\in C$.
Note that $\sum_{b_v} \weight(b_v)=O(n)$. 
\mdb{Add argument.}
Now compute a separator~$\sep^*$
of $\gpr(S^*\cup C)$ such that 
\[
\sum_{v\in \sep^*} (\log(\weight(v)) + 1 ) = O(\sqrt{n}).
\]
\mdb{Explain how to do this: take a set~$D$ of disks such that $\gpr(S^*\cup C)$ is the contact graph of the disks; duplicate the disk $\disk(v)$ corresponding to a node $v$ so that it has $\weight(v)$ copies; then apply the result of \cite{bbkmz-ethf-18}; and argue it works since each clique in $B$ corresponds to at most four nodes in $\gpr(S^*\cup C)$.}
We convert $\sep^*$ into a clique-based separator $\sep$ for $\ig(S)$ as follows.
\begin{itemize}
\item For each object $o_i^*\in\sep^*$ we put the object $o_i\in S$ into~$\sep$.
\item For each connector $b_v\in\sep^*$ we put the 
clique $S_v := \{ o_i : v\in \bd o^*_i \}$ into $\sep$.
\end{itemize}
\mdb{The fact that $v$ is used for nodes in $\gpr(S^*\cup C)$ and for a vertex
in the map is confusing.}
If an object is added multiple times, we remove all but one of its occurrences.

Clearly the weight of $\sep$ is as desired. We now prove the $\sep$ is a separator.
Let $A^*$ and $B^*$ be the two subsets of $S^*\cup C$ separated by $\sep^*$.
Thus $|A^*| \leq ...$ and $|B^*| \leq ...$,
    \mdb{add size}
and there are no edges from $A^*$ to $B^*$. 
Let $A := \{ o_i : o^*_i \in A^*\}$ and $B := \{ o_i : o^*_i \in B^*\}$
be the partition of $S\setminus \sep$ derived from $A^*,B^*$. 
The sets $A$ and $B$ have the desired size, so we only need to argue
that there are no edges form $A$ to~$B$. 

Consider a pair $(o_i,o_j)\in A\times B$. By definition of $A$ and $B$
we have $(o_i^*,o_j^*)\in A^*\times B^*$. Hence, $o_i$ and $o_j$ 
cannot be proper neighbors; otherwise $(o^*_i.o_j^*)$ is an edge in $\gpr(S^*\cap C)$,
which contradicts that $(o_i^*,o_j^*)\in A^*\times B^*$. The objects~$o_i$ and $o_j$ 
cannot be improper neighbors either. Indeed, in that case there would be a connector
$b_v$ such that $(o^*_i,b_v)$ and $(o^*_i,b_v)$ are edges in $\gpr(S^*\cup C)$.
But then we must have $b_v\in \sep^*$, which would imply that both $o_i$ and $o_j$
have been put into $\sep$.
\end{proof}
%--------------------------------------------------------------------------------------

==> OLD/other-stuff.tex <==
\mdb{Since pseudo-disks have linear union complexity, we can use the result from the previous section. Can be do better? Here's an idea that we had that  might be useful, although currently we do not see at all how to use this.}

Let $S$ be a collection of pseudo-disks, and assume without loss of generality that
$\ig(S)$ is connected. (If we can find a good separator for connected graphs, we
can also find good separators in the general case.)
\begin{lemma}
Suppose there is a simple closed curve~$\gamma$ with the following property:
There is a circular sequence $\Gamma := o_0,o_1,\ldots,o_{t-1},o_0$ of objects from $S$
such that $o_{i}\cap o_{(i+1)\mod t} \neq \emptyset$ for all~$0\leq i<t$---we call
such a sequence a \emph{necklace}---and $\gamma\subset \mbox{union}(\Gamma)$ and $\gamma$
visits the objects from $\Gamma$ in the given order.
\mdb{Not sure if this is the correct way of stating it. The idea is to have something
like in Fig.~\ref{fi:necklace}, though I think it might be okay if an object appears multiple times.}
Let $Q$ be the set of intersection points between the boundaries of consecutive objects in
the necklace, that is,
\[
Q := \{ \bd o_i \cap \bd o_{i+1} : 0\leq i < t \}.
\]
Then any object $o_j\in S$ that ``crosses from inside the necklace to outside the necklace"
contains at least one point from~$Q$.
\end{lemma}
%--------------------------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics{Figures/necklace.pdf}
\end{center}
\caption{A necklace and a curve $\gamma$ visiting the objects from the necklace in order.}
\label{fi:necklace}
\end{figure}
%--------------------------------------------------------------------------------------

==> OLD/pseudo-squares-old.tex <==
%--------------------------------------------------------------------------------------
\section{Pseudo-squares}
%--------------------------------------------------------------------------------------

%--------------------------------------------------------------------------------------
\begin{theorem}\label{th:pseudo-square-separator}
Let $S$ be a set of $n$ pseudo-squares in the plane. Then the intersection 
graph $\ig(S)$ has a clique-based separator of weight~$O(\sqrt{n}\log^4 n)$.
\end{theorem}
%--------------------------------------------------------------------------------------
\begin{proof}
Idea (if I remember correctly): 
\begin{enumerate}
\item Partition $S$ into a collection of cliques such that,       
      if you replace each clique by the union of its constituent pseudo-squares, the 
      set of these polygons has ply $O(\log^2 n)$.
      From each such clique select the at most four rectangles that are extreme in
      directions $+x,-x,+y,-y$. Let $R^*$ be the set of all extreme rectangles.
\item Consider the arrangement $\arr(R^*)$. Since the ply of $R^*$ is $O(\log^2 n)$
      and the rectangles in $R^*$ are pseudo-squares, $\arr(^*)$ has complexity
      $O(n\log^2 n)$. Construct a vertical decomposition of $\arr(R^*)$, and 
      consider its dual graph $\graph^*$. Since each vertex of the vertical decomposition
      has degree three or four, the faces in the dual graph are either triangles or
      quadrilaterals. Add an additional edge in each quadrilateral so we obtain a
      maximally planar graph. \mdb{Up to outer face}. 
\item Construct a separator $\sep^*$ for $\graph^*$ that is a cycle; such a separator
      exists since $\graph^*$ is maximally planar. It has $O(\sqrt{n\log^2 n} = O(\sqrt{n}\log n)$
      nodes. Each node is a face in the vertical decomposition. 
      Now construct the separator $\sep$ for $\ig(S)$: for each face $f\in \sep^*$
      and each rectangle $r\in R^*$ with $f\subset r$, add the clique of $r$ to $\sep$.
      Note that the weight of $\sep$ is 
      \[
      O(\sqrt{n}\log n) \cdot O(\log^2 n) \cdot O(\log n) = O(\sqrt{n} \log^4 n).
      \]
\item Construct the partition $A\cup B$ of $S\setminus \sep$, as follows.
      Let $A^*$ and $B^*$ be the two sets into which the node set of $\graph^*$
      are split by $\sep^*$. For any $r\in R^*\setminus \sep^*$, take an arbitrary face~$f$
      of the vertical decomposition contained in~$r$ and assign $r$ to $A$ iff $f$ is assigned to $A^*$.
      For each rectangle $r\in R\setminus (R^*\cup \sep)$ add $r$ the the same set as the
      extreme rectangles in its cliques. Argue that all of this is consistent, and argue
      that rectangles from $A$ cannot intersect rectangles from $B$.
      We also need to ensure the separator is balanced, which may require some extra work. 
\end{enumerate}
\end{proof}
%--------------------------------------------------------------------------------------

==> OLD/relation-between-classes.tex <==
%--------------------------------------------------------------------------------------
\section{Relation between graph classes}
%--------------------------------------------------------------------------------------

%--------------------------------------------------------------------------------------
\subsection{Map graphs are intersection graphs of fat objects}
%--------------------------------------------------------------------------------------
Let $S$ be a set of $n$ interior-disjoint objects in the plane.
We say that two objects from~$S$ are \emph{neighbors} if $\bd o_i\cap \bd o_j \neq \emptyset$.
We say that two neighbors $o_i$ and $o_j$ are \emph{proper neighbors} if $\bd o_i\cap \bd o_j$
has non-zero length; otherwise they are \emph{improper neighbors}.
Recall that the intersection graph $\ig(S)$ has an edge between two objects if and only
if they are neighbors. We define the \emph{proper intersection graph} of $S$,
denoted by $\gpr(S)$, to be the graph with node set $S$ where we only add edges
between proper neighbors. Since proper intersection graphs are planar, they are
more convenient to work with. Hence, we first describe a procedure that constructs,
given a set $S$, a set $S^*\cup C$ such that $\gpr(S^*\cup C)$ is a suitable representation of
$\ig(S)$.
\medskip

%--------------------------------------------------------------------------------------
%\paragraph{Regularization.}
%--------------------------------------------------------------------------------------
Let~$\subdiv(S)$ be the subdivision defined by~$S$.
Because we do not require the objects to have constant complexity, any two object 
boundaries can meet arbitrarily many times. As a result the number of vertices, 
edges and faces of~$\subdiv(S)$ need not be linear in~$n$. To avoid this, we 
first modify the objects from $S$, as follows. 

Let $H$ be the set of bounded faces of $\subdiv(S)$ whose boundary consists of 
boundary pieces of exactly two objects in~$S$. We add each face $f\in H$
arbitrarily to one of two objects contributing to its boundary.
Let $S^+$ be the resulting set of objects. Note that each object~in~$S$ is contained
in exactly one object in~$S^+$. Moreover, two objects $o_i,o_j\in S$ are neighbors
if and only if the corresponding objects in~$o^+_i,o_j^+\in S^+$ are neighbors:
proper neighbors stay proper neighbors, improper neighbors either stay improper
neighbors or become proper neighbors, and no new neighbors are introduced.

Now consider the subdivision~$\subdiv(S^+)$. Observe that $\subdiv(S^+)$ has a 
linear number of faces and, hence, a linear number of edges and vertices. 
    \mdb{Add argument}  
We say that a vertex~$v$ of $\subdiv(S^+)$ is \emph{irregular}
if there are at least two objects $o_i,o_j$ that touch at~$v$, meaning that in 
a sufficiently small neighborhood of~$v$ we have $\bd o_i \cap \bd o_j = v$;
see Fig.~\ref{fi:regularize} for an illustration. A vertex that is not
irregular is called \emph{regular}.
Let $\Vir$ be the set of non-regular vertices~of~$\subdiv(S^+)$. 
For an irregular vertex~$v$, let $S_v\subseteq S$ be the set of objects
whose boundary contains~$v$. For each irregular vertex~$v$, we place a small 
disk $b_v$ with its center at~$v$. The disks $b_v$ are chosen
small enough so that each disk~$b_v$ intersects only the objects in $S_v$;
it does not intersect any  no other objects from~$S$ nor any other disk~$b_{v'}$.
We call $b_v$ a \emph{connector}. Let $C := \{ b_v : v\in \Vir \}$
be the set of all connectors.
%--------------------------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics{Figures/regularize.pdf}
\end{center}
\caption{(i) A set $S$ of interior-disjoint objects, with non-regular vertices are shown in red.
           (ii) The regularization of $\ig(S)$ is shown in blue.
                The dark grey disks with a red boundary are the connectors.}
\label{fi:regularize}
\end{figure}
%--------------------------------------------------------------------------------------
For each object $o^+_i\in S^+$, we now define $o^*_i := o_i^+ \setminus \bigcup_{v\in \Vir} b_v$. 
Thus $o^*_i$ is obtained from~$o_i^+$ by removing the parts of $o_i^+$ inside the connectors
of its incident irregular vertices. Let $S^*$ be the resulting set of objects.
We summarize the important properties of the set~$S^*\cup C$.
\begin{itemize}
\item The total number of objects and disks in $S^*\cup C$ is $O(n)$.
\item Each object $o_i\in S$ corresponds to exactly one object in~$o^*_i\in S^*$.
\item If two objects $o_i,o_j\in S$ are proper neighbors then the corresponding
      objects $o^*_i,o^*_j\in S^*$ are proper neighbors.
\item If two objects $o_i,o_j\in S$ are improper neighbors then $o^*_i$
      and $o^*_j$ are proper neighbors or there is a connector
      $b_v\in C$ that is a proper neighbor of both~$o^*_i$ and $o^*_j$.
\item If $o^*_i,o^*_j\in S$ are neighbors, or $o^*_i$ and $o^*_j$
      have a connector $b_v$ as common neighbor, then $o_i,o_j$ are neighbors.
\end{itemize}
We call $\gpr(S^*\cup C)$ the \emph{regularization} of~$\ig(S)$. Using $\gpr(S^*\cup C)$
we can now easily prove the following theorem. Here we use the same definition 
of fat objects as De~Berg~\etal~\cite{bbkmz-ethf-18}. Namely, a planar object~$o$
is called $\alpha$-fat, for some $0<\alpha\leq 1$ if there are concentric disks~$b_\myin$ 
and $b_\myout$ such that $b_\myin \subseteq o \subseteq b_\myout$ and 
$\radius(b_\myin) /\radius(b_\myout) \geq \alpha$. We say that a set $F$ 
consists of fat objects if all objects in $F$ are $\alpha$-fat for some absolute
constant~$\alpha$. 
%--------------------------------------------------------------------------------------
\begin{theorem} \label{th:map-graph-to-fat}
Any map graph is the intersection graph of a set of $(1/5)$-fat objects in the plane.
\end{theorem}
%--------------------------------------------------------------------------------------
\begin{proof}
By definition, a map graph is the intersection graph~$\ig(S)$ of a set $S$ of~$n$
interior-disjoint objects in the plane. We need to show that there is a set~$F$
of fat objects such that $\ig(S)$ is isomorphic to $\ig(F)$. 

Let $\gpr(S^*\cup C)$ be the regularization of~$\ig(S)$. The graph $\gpr(S^*\cup C)$ 
is planar, so by the Koebe–Andreev–Thurston Theorem~\cite{koebe-36,thurston-78} it is the contact graph of 
a set of disks. In other words, there is a collection~$D$ of interior-disjoint disks, 
one for each element of $S^*\cup C$, such that $\gpr(S^*\cup C)$ is isomorphic to~$\ig(D)$.  
We denote the disk corresponding to an object $o^*_i\in S^*$ or a connector $b_v\in C$
by $\disk(o^*_i)$ and $\disk(b_v)$, respectively.

Now consider an object~$o_i\in S$. Let $\Vir(o_i)$ be the set of all irregular
vertices of~$\subdiv(S^+)$ on the boundary of~$o^+_i$, where $S^+$ and $o_i^+$
are defined as above, and let $C(o_i)\subseteq C$ be the connectors corresponding
to these irregular vertices. Define
\[
f_i := \ \ \disk(o^*_i) \ \cup \bigcup_{b_v\in C(o_i)} \disk(b_v),
\]
and set $F := \{ f_i : o_i \in S\}$.
Each $f_i\in F$ is the union of a central disk, $\disk(o^*_i)$, and zero or more
disks each touching the central disk. Hence, if $b_{\max}$ is a largest disk
among the disks comprising~$f_i$ then any point $p\in f_i$ is at distance at most
$5\cdot\radius(b_{\max})$ from the center of~$b_{\max}$. Thus $f_i$ is $(1/5)$-fat.
\medskip

To finish the proof it remains to argue that~$\ig(S)$ is isomorphic to~$\ig(F)$,
with the isomorphism that maps $o_i$ to~$f_i$. 

Let $(o_i,o_j)$ be an edge of~$\ig(S)$.
If $o_i$ and $o_j$ are proper neighbors then $o^*_i,o^*_j\in S^*$ are proper neighbors,
and so $(o_i,o_j)$ is an edge of~$\gpr(S^*\cup C)$. Hence, $\disk(o_i)$ touches $\disk(o_j)$
which implies that $f_i$ touches~$f_j$.
If $o_i$ and $o_j$ are improper neighbors then $o^*_i$ and $o^*_j$ are proper neighbors
or there is a connector
$b_v\in C$ that is a proper neighbor of both~$o^*_i$ and $o^*_j$. In the former case
$f_i$ touches $f_j$, as before. In the latter
case $\disk(b_v) \subset f_i$ and $\disk(b_v) \subset f_i$, implying that
$f_i$ intersects~$f_j$. In all cases  $(f_i,f_j)$ is an edge of~$\ig(F)$.

Conversely, consider an edge $(f_i,f_j)$ of~$\ig(F)$. Then either $f_i$ and $f_j$
some~$\disk(b_v)$ in common, where $b_v$ is a connector, or $f_i$ and $f_j$ touch.
In the former case, $o_i$ and $o_j$ share an irregular vertex. 
In the latter case, $\disk(o^*_i)$
and $\disk(o^*_j)$ must touch. (Indeed, connectors are disjoint and so their
representative disks in $D$ are disjoint as well, and whenever some $\disk(b_v)\in D$
touches some $\disk(o^*_i)$ than $\disk(b_v)$ is added to~$f_i$.)
In both cases $(o_i,o_j)$ is an edge of~$\ig(S)$.
\end{proof}
%v--------------------------------------------------------------------------------------

==> app-missing-proofs.tex <==
%------------------------------------------------------------------------------------------
\section{Omitted lemmas and proofs}
\label{app:missing-proofs}
%------------------------------------------------------------------------------------------

%------------------------------------------------------------------------------------------
\begin{lemma}\label{le:map-graph-separator-sep}
There are no arcs in $\ig(F)$ between a node in $A$ and a node in $B$.
\end{lemma}
%------------------------------------------------------------------------------------------
\begin{proof}
Suppose for a contradiction that there are objects $f\in A$ and $f'\in B$
such that $(f,f')$ is an arc in $\ig(F)$. Let $q\in Q$ be a witness point for the 
arc~$(f,f')$; thus $(p_f,q)$ and $(p_{f'},q)$ are arcs in~$\myH_1$. 
Consider the gadget~$G_q$ and the tree~$\tree_q$. Let $\pi$ denote
the path from $p_f$ to $p_{f'}$ in $\tree_q$. Note that none of the nodes on $\pi$ 
can be in~$\sep(\myH_2)$, otherwise $V_q$ contains an ancestor of $p_f$ or of $p_{f'}$,
and (at least) one of the nodes $p_f,p_{f'}$ is in a clique that was added to $\sep$.
But then the nodes $p_f,p_{f'}$ are still connected in $\myH_2$ after the removal
of~$\sep(\myH_2)$. Hence, we have $p_f,p_{f'} \in A(\myH_2)$ or $p_f,p_{f'} \in B(\myH_2)$,
both contradicting that $f\in A$ and $f'\in B$.
\end{proof}
%--------------------------------------------------------------------------------------

%--------------------------------------------------------------------------------------
\begin{lemma}
\label{le:connected}
Let $D^*_i,D^*_j\in\D^*$.
Every connected component of $D_i^* \setminus D_j^*$ contains a point $u$ with $u\in D_i \setminus D_j$.
\end{lemma}
%--------------------------------------------------------------------------------------
\begin{proof}
The only case of interest is when there exist $\gamma_i \in \Gamma(D_i)$ and 
$\gamma_j \in \Gamma(D_j)$ such that $\gamma_i \cap \gamma_j \neq \emptyset$.
Suppose now there is a connected component of $D_i^* \setminus D_j^*$ which does not contain 
such a point. Since $D_i^*\subset D_i$ and $D_j^* \subset D_j$, this connected component must 
have been introduced due to the perturbation  (in other words its intersection with all 
connected components of $D_i\setminus D_j$ must be empty). This means that this connected component 
must be the region contained between $\gamma_i^*$ and $\gamma_j^*$  and which was 
previously contained in $D_i \cap D_j$. It is enough to only examine the case when $\gamma_i$ is 
bigger than $\gamma_j$ as otherwise this component only contains points of $D_j^*$. 
There are two cases: $\gamma_j\subset \gamma_i$, or $\gamma_j \not \subset \gamma_i$. 
In both cases note that there will exist an endpoint $p$ of $\gamma_j^*$ that lies inside $D_i^*$. 
Choose now a point $q$ in $(D_j\setminus D_j^*) \setminus (D_i\setminus D_i^*)$ at 
distance $\eps$ from $\gamma_j$ with $\eps_{\gamma_i} < \eps < \eps_{\gamma_j}$. 
See Fig.~\ref{fi:perturbation-proof} for an illustration of the case $\gamma_j\subset \gamma_i$. 
Consider the dashed path starting at $q$ that stays at distance~$\eps$ from $\bd P$
going towards~$p$. Due to the definition of our perturbation this path 
will stay inside $D^*_i$ and remain outside $D_j^*$. Hence, after exiting $D^*_j$
near the point $p$ we reach a point $u \in D_i \setminus D_j$, which is
a contradiction.
\end{proof}
%------------------------------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics{Figures/perturbation-proof.pdf}
\end{center}
\caption{Illustration for proof of Lemma 19.}
\label{fi:perturbation-proof}
\end{figure}
%------------------------------------------------------------------------------------------

==> app-vis-graph.tex <==
%--------------------------------------------------------------------------------------
\section{A clique-based separator for visibility-restricted unit-disk graphs}
\label{app:vis-graph}
%--------------------------------------------------------------------------------------

%--------------------------------------------------------------------------------------
\subsection{Centerpoint of a simple polygon}
\label{app:centerpoint}
%--------------------------------------------------------------------------------------
Here we introduce the concept of a centerpoint inside a simple polygon~$P$. 
This is a natural extension of the notion of the centerpoint for 
a set $Q$ of $n$ points in the plane, which is a point~$p$ (not necessarily from $Q$) such that
any line through~$p$ divides the plane in two half-planes each containing at most $2n/3$ 
of the points from~$Q$. Recall that a \emph{chord} in $P$ is a line segment $s\subset P$ that connects
two points on the boundary of~$P$. Since we consider $P$ to be a closed set,
a chord may pass through one or more reflex vertices of~$P$.
We say that a chord is \emph{maximal} if it cannot be extended without exiting the polygon.
We define a \emph{half-polygon} of $P$ to be a sub-polygon of $P$ that is bounded by
a (not necessarily maximal) chord~$s$ and a portion $\gamma\subset \bd P$ of the boundary of $P$
such that $s\cap \gamma=\{z_1,z_2\}$, where $z_1,z_2$ are the endpoints of~$s$.
Note that any chord splits $P$ into two or more half-polygons.
%--------------------------------------------------------------------------------------
\begin{definition}[Centerpoint in a Simple Polygon]
Let $P$ be a simple polygon and $Q$ be a set of $n$ points in $P$. 
A \emph{centerpoint for $Q$ in $P$} is a point $p\in P$ such that any maximal chord through $p$ 
splits $P$ into half-polygons that each contain at most $2n/3$ points from $Q$ in their interior. 
\end{definition}
%--------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------
\begin{theorem} \label{th:centerpoint}
For any simple polygon $P$ and point set $Q\subset P$,  a centerpoint for $Q$ in $P$ exists.
% \mdb{time to find it?}
\end{theorem}
%--------------------------------------------------------------------------------------
\begin{proof}
To prove the theorem we can follow the standard proof~\cite{m-lecture-notes} of the existence of a centerpoint in the plane
almost verbatim.
Thus, consider the family $H$ of all half-polygons of $P$ whose interior contains more than $2n/3$ points of~$Q$. 
Any three of these half-polygons must intersect, because the complement of each of them contains 
less than $n/3$ points from~$Q$. Recall that Helly's Theorem states that if we have a family
of convex sets in the plane such that any three of them intersect, then they all intersect in
a common point. While our half-polygons are not convex, the same result is true here, as follows
from Molnar's Theorem ~\cite{Breen98} which states that if a family of simply connected compact sets 
in the plane is such that any two members have a connected intersection and any three members 
have a non-empty intersection, then the intersection of the family is non-empty. 
Our family $H$ satisfies these conditions and hence $\bigcap H \neq \emptyset$.

We claim that any point $c$ in the common intersection of the half-polygons in $H$ is a centerpoint
for $Q$ in $P$. To see this take a chord~$s$ through $c$ and let $H_1,H_2,\ldots$ be the
half-polygons into which $s$ splits~$P$. Suppose for contradiction that some $H_i$ contains more than $2n/3$ points of $Q$. 
Let $s_i\subseteq s$ be the part of~$s$ bounding~$H_i$.
Then, if we slightly shrink $H_i$ by moving~$s_i$ infinitesimally, we obtain a half-polygon~$H'_i$
that contains more than~$2n/3$ vertices, contradicting the definition of~$c$.
\end{proof}


%--------------------------------------------------------------------------------------
\subsection{The separator construction in a simple polygon}
\label{app:vis-graph-simple}
%--------------------------------------------------------------------------------------
Our separator construction has two steps. In the first step we put all points that can see
a reflex vertex within distance~$\sqrt{2}$ into the separator. We will argue that we
can do this in such a way that we put $O(1)$ cliques per reflex vertex into
the separator. In the second step we handle the remaining points. We take a centerpoint~$c$
inside~$P$ and then define $\sqrt{n}$ chords through~$c$. For each chord~$s_i$ we put the
points within distance~1/2 into the separator, suitably grouped into cliques. We will argue that
the total weight of the cliques, over all chords~$s_i$ is $O(n)$.
Hence, the there is a chord whose cliques have total weight $O(\sqrt{n})$.
Adding the weight of the cliques we added in Step~1 then gives us the desired separator.


%--------------------------------------------------------------------------------------
\paragraph*{Step~1: Handling points that see a nearby reflex vertex} 
%--------------------------------------------------------------------------------------
Let $\Vr$ be the set of reflex vertices of $P$, and let $Q_1\subseteq Q$ be the set 
of points that can see a reflex vertex within distance~$\sqrt{2}$. 
Consider the geodesic Voronoi diagram of $\Vr$ within~$P$. Let $R(u)$ be the Voronoi region of 
vertex $u\in \Vr$ and define $R^*(u) := R(u) \cap D(u,\sqrt 2)$. 
% where $D(u,\sqrt2 )$ denotes the disk centered at $u$ with radius $\sqrt 2$.
Note that all points in $R(u)$ can see~$u$ and that all points in $Q_1$ are in~$R*(u)$ for
some vertex~$u\in \Vr$. The following lemma is illustrated in Fig.~\ref{fi:vis-lower-bound}(ii)
in the main text.
%--------------------------------------------------------------------------------------
\begin{lemma} \label{le:split-Rstar}
Let $e$ be an edge incident to $u$. If we extend $e$ until it hits $\bd R^*(u)$
then $R^*(u)$ is split into two convex parts.
\end{lemma}
%--------------------------------------------------------------------------------------
\begin{proof}
It suffices to argue that the angle of $R(u)$ corresponding to $u$ is the only reflex angle within $R(u)$. 
Then the result will follow from the fact that $D(u,\sqrt 2)$ is convex. Clearly the shortest path connecting 
any point $p \in R(u)$ to $u$ is the segment~$pu$. This implies that $\bd R(u)$ consists of 
straight line segments that are parts of perpendicular bisectors of the segments connecting 
$u$ to other reflex vertices of $P$. Any two such consecutive edges then cannot form a reflex angle within $R(u)$.
\end{proof}
%--------------------------------------------------------------------------------------
Since $R^*(u)$ has diameter~$O(1)$, Lemma~\ref{le:split-Rstar} implies that $Q_1\cap R^*(u)$ 
can be partitioned into $O(1)$ cliques. We collect all these cliques into a set~$\sep_1$.
Since there are~$r$ reflex vertices, $\sep_1$ consists of $O(r)$ cliques whose total
weight is~$O(r\log(n/r))$.  


%--------------------------------------------------------------------------------------
\paragraph*{Step~2: Handling points that do not see a nearby reflex vertex}
%--------------------------------------------------------------------------------------
%Let $c$ be the centerpoint of $P$. The idea is to draw $\sqrt n$ lines through the centerpoint and show how we can split points close to these lines into cliques of total weight $O(n)$. Then there will exist a line whose cliques will have a total weight of $O(\sqrt n)$. Note that the set of cliques that corresponds to each line will be a separator for the set $H$. 
%
%Let $m=\floor{\sqrt n}$. We draw $m$ lines $l_1,l_2,...,l_m$ through $c$ such that $l_1$ forms an angle of $\frac{\pi}{m}$ with the horizontal line through $c$ and $l_i$ forms an angle of $\frac{\pi}{m}$ with $l_{i+1}, i=1,...,m-1$. We also draw a grid of unit squares , with dimensions $(2m+1) \times (2m+1)$ with its central unit square centered at $c$. (see Fig. ~\ref{fig:square-grid}).  We will denote with $C_l$ the set of cliques that the separator corresponding to $l$ will contain. Note that $C_l$ now only contains points from the set $H$. We will denote with $\weight(C_l)$ the total weight of the cliques in $C_l$, that is: $$\weight(C_l)=\sum_{C \in C_l} \log{\left( |C|+1\right)}$$. 
%
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{Figures/square-grid.pdf}
%    \caption{The square grid centered at the centerpoint $c$ and the lines passing through $c$ for $m=6$.}
%    \label{fig:square-grid}
%\end{figure}
Our separator $\sep$ consists of the cliques in $\sep_1$ plus a set $\sep_2$
of cliques that are found as follows. 
Let $Q_2 := Q\setminus Q_1$ be the set of points that do not see a reflex vertex within distance~$\sqrt{2}$. 
Let $c$ be a \emph{centerpoint for $Q_2$ inside $P$},
that is, a point such that any chord through~$c$ splits~$P$ into two half-polygons containing 
at most $2|Q_2|/3$ points from $Q$.
Such a point exists by Theorem~\ref{th:centerpoint}.
Let $G$ be a $\sqrt{n}\times\sqrt{n}$ grid centered at~$c$,
where we assume for simplicity that $\sqrt{n}$ is integer. 
For each of the $\sqrt{n}$ points~$g_i$ in the rightmost column
of the grid (even if $g_i\not\in P$), we define a maximal chord~$s_i$ by taking the line~$\ell_i$ through $c$ and $g_i$
and then taking the component of $\ell_i\cap P$ that contains~$c$; see Fig.~\ref{fi:vis-separator-app}(i).
We assume for simplicity that the chords~$s_i$ doe not pass through reflex vertices;
this can be ensured by slightly rotating the grid, if necessary.

For each chord~$s_i$, we define $Q_2(s_i)$ be the set of points $q\in Q_2$
such that there is a point $z\in s_i$ that sees $q$ with $|qz|\leq 1/2$.
%--------------------------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics{Figures/vis-separator.pdf}
\end{center}
\caption{(i) The grid $G$ defining the chords~$s_i$. 
          (ii) The points in the top-left cell do not see each other, but they see a reflex vertex
               and so they are not in $Q_2(s_i)$.
               The points in the top-right cell can be partitioned into $O(1)$ cliques.}
\label{fi:vis-separator-app}
\end{figure}
%--------------------------------------------------------------------------------------
Note that $\gvis(Q)$ cannot have an arc between a point $p\in Q_2 \setminus Q_2(s_i)$ above $s_i$
and a point $q\in Q_2 \setminus Q_2(s_i)$ below $s_i$; otherwise $p$ and/or $q$ see a point on
$z$ within distance~1/2, and so at least one of $p,q$ is in $Q_2(s_i)$. Since $s_i$ is a chord
through the centerpoint~$c$, this means that $s_i$ induces a balanced separator.

It remains to argue that at least one of the chords~$s_i$ induces a separator whose weight
is small enough. We will do this by creating a set~$\sep(s_i)$ of cliques for each chord~$s_i$,
and prove that the total weight of these cliques, over all chords $s_i$, is $O(n)$. Since there
are $\sqrt{n}$ chords, one of them has the desired weight. 

%--------------------------------------------------------------------------------------
\mypara{Step~2.1: Points outside the grid.}
%--------------------------------------------------------------------------------------
We simply  put all points from $Q_2(s_i)$ that lie outside the grid $G$---that is, the points
that do not lie inside a grid cell---into $\sep(s_i)$, as singletons.
%--------------------------------------------------------------------------------------
\begin{observation}\label{obs:outside-grid}
Let $q$ be a point that does not lie in any of the cells of the grid~$G$. Then $q$ lies within
distance~$1/2$ of at most two chords~$s_i$.
\end{observation}
%--------------------------------------------------------------------------------------
%
% OLD PROOF< WITH DIFFERENT DEF OF GRID
%
%Let $p$ be a point which lies at distance greater than $\sqrt n$ from $c$. Let $vdist(p,l)$ (from \emph{visibility distance}) denote the distance of $p$ from its closest visible point on $l$.
%
%If $p$ lies on one of our lines, then it will have a visibility distance which is greater than $1$ from other lines. Obviously it suffices to show this for one of the two neighboring lines. 
%For the following refer to Fig. ~\ref{fi:farpoints}.
%
%We have that: $$\sin{\phi}=\frac{d}{r} \Leftrightarrow d=r\sin{\phi} >\sqrt n \sin{\frac{\pi}{\sqrt n}} $$
%
%\begin{figure}
%    \centering
%   \includegraphics[scale=0.7]{Figures/farpoints.pdf}
%    \caption{The circle of radius $m=\floor{\sqrt n}$ and center $c$ is drawn. Point $p$ lies outside this circle.}
%    \label{fi:farpoints}
%\end{figure}
%
%It's trivial to see that $\sqrt n  \sin{\frac{\pi}{\sqrt n}} >1 $ when $\sqrt n >=2$. Because $vdist(p,l)\geq d$,  we have that $vdist(p,l)> 1$. Therefore we can add such points to the separator of the line they lie on,  as singletons. 
%
%We similarly show that when $p$ lies between two lines then its distance from the next two closest lines is greater than $1$ and therefore it suffices to add it as a singleton to the separator of at most two lines. This shows that points that have a distance greater than $\sqrt n$ from $c$ add a total weight which is at most $2n$ to our separators. 
%
%--------------------------------------------------------------------------------------
Observation~\ref{obs:outside-grid} implies that the total number of singleton cliques
of points outside grid cells, summed over all chords~$\sep(s_i)$, is~$O(n)$.

%--------------------------------------------------------------------------------------
\mypara{Step ~2.2: Points inside the grid.}
%--------------------------------------------------------------------------------------
Next, consider a cell~$T$ of the grid $G$. Suppose a point $q\in Q_2(s_i)$ sees a point $z\in T\cap s_i$ 
such that $|qz|\leq 1/2$. Then $q$ must lie inside one of the at most nine grid cells surrounding and including~$T$.
Consider such a cell $T'$. 
%--------------------------------------------------------------------------------------
\begin{lemma}\label{le:inside-grid}
The points from  $Q_2(s_i)\cap T'$ that can see a point on $s_i\cap T$ within distance $1/2$ can be partitioned
into $O(1)$ cliques.
\end{lemma}
%--------------------------------------------------------------------------------------
\begin{proof}
We will show that we can split these points into at most four cliques. 
To this end we split $T'$ in four equal-sized subcells; see Fig.~\ref{fi:inside-grid}. 
Clearly each subcell has a diameter~$\frac{1}{2}\sqrt{2}<1$. It suffices now to show that if two points 
$p,q$ in the same subcell do not see each other, then they see a reflex vertex within distance $\sqrt 2$; 
hence they are in $Q_1$ and not in $Q_2(s_i)\cap T'$.
%--------------------------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics{Figures/inside-grid.pdf}
\end{center}
\caption{Illustration for the proof of Lemma~\ref{le:inside-grid}.}
\label{fi:inside-grid}
\end{figure}
%--------------------------------------------------------------------------------------

Let $z_1$ and $z_2$ be points on $s_i \cap T$ that see $p,q$, respectively, with
$|pz_1|\leq 1/2$ and $|qz_2| \leq 1/2$. The quadrilateral formed by the points $p,q,z_1,z_2$ must always lie 
within a square of side length~1. This square is shown in green in Fig.~\ref{fi:inside-grid}, for three different  
cases depending on the relative position of~$T'$ and~$T$. In this quadrilateral, the side~$pq$ has to be crossed 
by the $\bd P$, since we assumed $p$ and $q$ do not see each other. Moreover,
$\bd P$ cannot cross $s_i$ or the segments $pz_1,qz_2$. Thus at least one reflex vertex of $\bd P$
lies within the quadrilateral. It's then clear that both $p,q$ will be able to see a reflex vertex 
within the quadrilateral (possibly not the same); since all points lie within a square of diameter~1, 
the result follows. Note that in Fig.~\ref{fi:inside-grid} (iii) we have made the edges $pz_1,qz_2$ 
cross each other to showcase that the proof still goes through in this case.
\end{proof}
%--------------------------------------------------------------------------------------
We thus create $O(1)$ cliques for each cell~$T'$ that is one of the at most nine cells
surrounding a cell $T$ crossed by~$s_i$, and put them into~$\sep(s_i)$.
This adds at most $O(\log (n_{T'}+1))$ weight to $\sep(s_i)$, where $n_{T'} := |Q_2\cap T'|$.
Since there are $n$ cells in total, this immediately gives a total weight of
$O(n\log n)$ over all sets $\sep(s_i)$. Next we show that the the total weight of the cliques is actually $O(n)$. 
In what follows we denote by $\weight(\sep(s_i))$ the total weight of the cliques corresponding to chord $s_i$.
%--------------------------------------------------------------------------------------
\begin{lemma}
The total weight of the cliques corresponding to the chords $s_i$ is $O(n)$, that is:
\[
\sum_{i=1}^{\sqrt{n}}\weight(\sep(s_i))=O(n).
\]
\end{lemma}
%--------------------------------------------------------------------------------------
\begin{proof}
Let $\T(s_i)$ denote the cells crossed by a chord~$s_i$, and let $N[T]$ denote the at most
nine cells surrounding a cell~$T$, including $T$ itself.
By the arguments above, the total weight of all separators is.
%
\begin{equation}\label{eq:sum1}
\sum_{i=1}^{\sqrt{n}} \sum_{T\in\T(s_i)} \sum_{T'\in N[T]} O(\log (n_{T'}+1))
\end{equation}
%
Let $K_1$ be the set of cells in the central column of the grid, that is, the
column containing the centerpoint~$c$. For $2\leq j\leq m$, where $m:=\lceil \sqrt{n}/2\rceil,$
let $K_j$ be the cells in the pair of columns at distance~$j-1$ from~$K_1$.
For example, $K_2$ are the cells in the columns immediately to the left and right of $K_1$.
Then we can make the following observations.
%
\begin{itemize}
\item The set~$K_j$ contains $4j-2=O(j)$ cells that are crossed by at least one chord~$s_j$.
\item Cells in $K_j$ are crossed by $O(\sqrt{n}/j)$ chords.
\end{itemize}
%
Now define $K^*_j$ to be the set of cells $T'$ in $K_j$ such that one of the nine cells
surrounding $T'$ is crossed by at least one chord. Note that each $T'\in K^*_j$
is in $N[T]$ for at most nine cells~$T$, which are all in $K_{j-1}\cup K_j\cup K_{j+1}$.
(Here we define $K_{-1}=K_{m+1}=\emptyset$.)
It then follows from the above observations that $|K_j^*|=O(j)$. Moreover, if
$T'\in K^*_j$ and $T'\in N[T]$, then $T$ is crossed by~$O(\sqrt{n}/j)$ chords.
Hence, we can rewrite~(\ref{eq:sum1}) as
\begin{equation}\label{eq:sum2}
\sum_{j=1}^{m} \left( O\left(\frac{\sqrt{n}}{j}\right) \cdot \sum_{T'\in K^*_j} O(\log (n_{T'}+1)) \right)
=
O\left( \sum_{j=1}^{m}  \frac{\sqrt{n}}{j} \cdot \sum_{T'\in K^*_j} \log (n_{T'}+1) \right)
\end{equation}
Now we are ready to compute the total weight of the separator. Note that
\[
\sum_{T'\in K^*_j} \log (n_{T'}+1) =   \log \left( \prod_{T'\in K^*_j} (n_{T'}+1)) \right)
\]
Now define $n_j$ to be the total number of points in the cells in $K^*_j$.
The AM-GM inequality gives us:
\[
\log \left( {\prod_{T' \in K^*_j }(n_{T'}+1)} \right)
\leq \log \left( \left(\frac{\sum_{T'\in K^*_j} (n_{T'}+1)}{|K_j^*|}\right)^{|K_j^*|} \right)
= |K_j^*| \log \left( \frac{n_j}{|K^*_j|} + 1 \right),
\]
Since $|K^*_j| = O(j)$ we have 
\[
|K_j^*| \log \left( \frac{n_j}{|K^*_j|} + 1 \right) =O\left( j\cdot \log \left(\frac{n_j}{j}+1\right)\right)
\]
Combining this with the previous we conclude that the total weight
over all separators is bounded by
\begin{equation} \label{eq:sum3}
O\left( \sum_{j=1}^{m}  \frac{\sqrt{n}}{j} \cdot j \log \left( \frac{n_j}{j} + 1 \right) \right)
=
O\left( \sum_{j=1}^{m}  \sqrt{n} \cdot \log \left( \frac{n_j}{j} + 1 \right) \right)
\end{equation}
We have that: 
\begin{equation}\label{eq:sum4}
\sum_{j=1}^{m} \log \left( \frac{n_j}{j} + 1 \right) 
=
O\left(\log \left( \frac{\prod_{j=1}^{m} n_{j}}{ m !}\right)\right)
\end{equation}
Recall that $m=\lceil \sqrt{n}/2 \rceil$, which implies that $n/m \leq 2m$.
Furthermore, Stirling's approximation tells us that $\log (m!) = m\log m - m + O(\log m)$.
Since $\sum_{j=1}^m n_j \leq n$ and using the AM-GM inequality we derive
\[
\begin{array}{lll}
\log \left( \frac{\prod_{j=1}^{m} n_{j}}{ m !} \right) &
\leq &
\log \left( (n/m)^m \right) - \log (m!) \\
& = & m \log (n/m) -  \left( m\log m - m + O(\log m) \right) \\
& \leq & m \log (2m) - \left( m\log m - m + O(\log m) \right) \\
& = & 2m + O(\log m) \\
& = & O(\sqrt{n})
\end{array}
\]
Combing this with Equations~(\ref{eq:sum3}) and~(\ref{eq:sum4})
we conclude that the total weight of the sets $\sep(s)$ is $O(n)$, as claimed.
\end{proof}
%--------------------------------------------------------------------------------------
We conclude that there will be a chord $s_i$ whose cliques have total weight $O(\sqrt n)$. Then our desired separator is the set $\sep=\sep_1 \cup \sep(s_i)$.


%--------------------------------------------------------------------------------------
\subsection{Extension to polygons with holes}
%--------------------------------------------------------------------------------------
We now show how to extend the previous approach so that it also works for a polygon~$P$ 
with holes. The key ideas remain the same. 
\medskip

As previously, the first step is to put the points that see a reflex vertex within distance $\sqrt 2$
into the separator. This can again be done using the geodesic Voronoi diagram of the reflex vertices. 
Recall that a vertex of a hole is defined to be reflex if its angle within $P$ (not: within the hole) 
is more than 180~degrees.
\medskip

In the second step we again construct $\sqrt{n}$ potential separators. When $P$ has holes, a chord
may not split $P$ into two half-polygons. Hence, instead of taking chords though a centerpoint 
for~$Q_2$ in~$P$, we proceed slightly differently. We take
a regular centerpoint for~$Q_2$, and for each point~$g_i$ in the rightmost column of
the grid~$G$ we take the full line~$\ell_i$ through $c$ and~$p_i$. Note that $\ell_i\cap P$ 
can consist of many chords. Together, these chords split $P$ into several parts; the parts 
above~$\ell_i$ contain at most $2|Q_2|/3$ points, and the parts below $\ell_i$ contain at most $2|Q_2|/3$ points as well.
Hence, the resulting separators will be balanced.

Points in $Q_2$ that lie outside the grid~$G$ can be handled as before. They are added as 
a singleton to $O(1)$ lines~$\ell_i$, so they contribute weight $O(n)$ in total.

%--------------------------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics{Figures/holes.pdf}
\end{center}
\caption{A line $\ell_i$ which crosses a cell $T$ that has three holes, colored in red. The blue piece of $\ell_i$ is the entrance piece, while the two green pieces are the non-entrance pieces. Note that each green piece can be uniquely associated to the pair of entrance-exit points of the hole preceding it. Marked with a cross are two possible choices of reflex vertices that are then associated with the green pieces.}
\label{fi:holes}
\end{figure}
%--------------------------------------------------------------------------------------
We now proceed to describe how to split points in $Q_2$ within the grid into cliques.  
For each line $\ell_i$ and each grid cell $T$ we define an \emph{entrance piece} to be 
the first piece of $\ell_i \cap T \cap P$. The remaining pieces will be referred to as 
\emph{non-entrance pieces} (see Fig.~\ref{fi:holes}). Entrance pieces can be handled 
exactly as in the case without holes: we look at all the points in the nine cells 
surrounding and including $T$ which see this piece within a distance $1/2$ and split 
them in a constant number of cliques. Then the total sum of the weights of these 
cliques for all the lines will be $O(n)$ as before. Thus we can select a line~$\ell_i$ 
such that the weight of the cliques we add for their
for the entrance pieces is $O(\sqrt{n})$. 

It remains now to handle the non-entrance pieces. Let~$\ell_i$ be the line we
selected. We will show that $\ell_i$ 
has $O(r)$ non-entrance pieces and that for each of them we only need to add $O(1)$ cliques. 
For the first part, observe that if a line $\ell_i$ intersects a hole $2k$ times then 
the hole must have at least $k$ reflex vertices of $P$. These $2k$ points of intersection 
can be split into $k$ pairs of entrance-exit points. Now note that a non-entrance piece can be 
uniquely associated with a unique pair of entrance-exit points. Therefore we have associated 
each non-entrance piece with a unique reflex vertex of $P$ and as a result the number of these pieces is indeed $O(r)$.
The second part is handled as before by adding a constant number of cliques from the nine cells that surround the cell that contains each non-entrance piece.
Therefore the cliques that correspond to these pieces add a total weight of $O(r \log \frac{n}{r})$. 

To summarize, after having found a separator such that the total weight of the entrance pieces is $O(\sqrt{n})$
we can add the cliques for the  non-entrance pieces to obtain a separator of weight $O(r \log \frac{n}{r}+\sqrt n)$.
Together with the cliques from $\sep_1$ this gives the final separator.
This finishes the proof of Theorem~\ref{th:vis-separator}.




==> sec-preliminaries.tex <==
%--------------------------------------------------------------------------------------
\section{Preliminaries}
%--------------------------------------------------------------------------------------
The classic Planar Separator Theorem as stated above says that any planar graph admits 
a separator of size $O(\sqrt{n})$ such that the parts induced by the separator have 
at most $2n/3$ nodes. The original statement is actually a bit more general: one can
assign each node a non-negative cost such that $\sum_{v\in V}\cost(v)=1$ and then the
parts induced by the separator have total cost at most~$2/3$. We need an even more general
version, where each node also have an integer weight and the ``size'' of the separator
is defined to be $\sum_{v\in \sep} \log (\weight(v)+1)$.
%--------------------------------------------------------------------------------------
%\begin{theorem}\label{th:weight-balanced-planar-separator}
%Let $\graph=(V,E)$ be a planar graph with $n$ vertices, where each vertex $v\in V$ 
%has a non-negative cost, denoted~$\cost(v)$, such that $\sum_{v\in V}\cost(v)=1$. Then $V$ can
%be partitioned into three sets $A,B,\sep$ such that 
%\begin{itemize}
%\item There are no edges in $E$ between a vertex in $A$ and a vertex in $B$.
%\item The separator is balanced with respect to the vertex costs: 
%      $\sum_{v\in A} \cost(v) \leq 2/3$ and $\sum_{v\in B} \cost(v) \leq 2/3$.
%\item The separator size is small: $|\sep| = O(\sqrt{n})$
%\end{itemize}
%The separator $\sep$ and sets $A$ and $B$ can be found in \mdb{Add time bound.}
%\end{theorem}
%--------------------------------------------------------------------------------------

%--------------------------------------------------------------------------------------
\begin{theorem}\label{th:log-weighted-planar-separator}
Let $\graph=(V,E)$ be a planar graph with $n$ vertices, where each vertex $v\in V$ 
has positive integer weight such that $\sum_{v\in V}\weight(v)=W$
and a non-negative cost such that $\sum_{v\in V}\cost(v)=1$.
Then $V$ can be partitioned into three sets $A,B,\sep$ such that 
\begin{itemize}
\item There are no edges in $E$ between a node in $A$ and a node in $B$.
\item The separator is balanced with respect to the costs of the vertices:
      $\sum_{v\in A} \cost(v) \leq 36/37$ and $\sum_{v\in B} \cost(v) \leq 36/37$.
\item The weights of the nodes in of the separator satisfies $\sum_{v\in \sep} \log (\weight(v)+1) = O(\sqrt{W})$
\end{itemize}
The separator $\sep$ and sets $A$ and $B$ can be found in polynomial time. \mdb{Add time bound.}
\end{theorem}
%--------------------------------------------------------------------------------------
\begin{proof}
Recall that the graph $G$ can be realized as the intersection graph of a set~$F$ of
disks. Such a set~$F$ can be computed in polynomial time.
\mdb{We should look into this more closely. Dong~\etal~\cite{DongLQ20} showed something
along these lines, but they only give an approximate solution and their bound is randomized.}
Let $D_v$ be the disk representing node~$v\in V$. We generate $\weight(v)$ copies of
each disk~$D_v$; one of these copies gets cost~$\cost(v)$, the other copies get cost~zero.
This way we generate a set~$\D$ of $W$ disks in total, whose costs sum to~1.
We can now essentially follow the proof of De~Berg~\etal~\cite{bbkmz-ethf-20} that shows 
that any collection of $W$ disks has a balanced clique-based separator of weight~$O(\sqrt{W})$,
as explained next. 

The proof in~~\cite{bbkmz-ethf-20} starts by finding a smallest square~$H_0$ containing at least
$n/37$ of the disks. We modify this step and start with a smallest square such that
the total cost of the disks inside~$H_0$ is at least~$1/37$. Assume without loss of generality
that the edge length of~$H_0$ is~1. The proof then proceeds as follows. Let 
$H_1,\ldots,H_m$ be a collection of $m := \sqrt{n}$ squares with the same center as~$H_0$ and such that $H_i$ 
has edge length $1 + 2i/m$. Note that $H_m$ has edge length 3. 
We call a disk \emph{large} if its diameter is at least~$1/4$ and \emph{small} otherwise.
Let $\D_{\mylarge}$ denote the set of all large disks that intersect~$H_m$, and let 
$\D_{\bd}(H_i)$ denote the set of all disks intersecting~$\bd H_i$.
Each square~$H_i$ defines a possible separator, namely $\D_{\bd}(H_i)\cup \D_{\mylarge}$. 
In~\cite{bbkmz-ethf-20} it is argued that each~$H_i$ induces a balanced separator. 
More precisely, their argument implies that the number of disks
inside $H_i$ that are not in the separator, as well as the number of disks outside
$H_i$ that are not in the separator, is at most~$36n/37$. With our modified definition
of $H_0$, the argument gives us that the total cost of the disks inside $H_i$, as well as
the total cost of the disks outside~$H_i$, is at most~$36/37$.

Finally, the proof in~\cite{bbkmz-ethf-20} shows that there must be a square~$H_i$ such
that the separator $\D_{\bd}(H_i)\cup \D_{\mylarge}$ can be partitioned into a collection
$\C_i$ of cliques such that $\sum_{C\in \C_i}\log(1+|C|)=O(\sqrt{|\D|})=O(\sqrt{W})$. 
We now observe that (i) the cliques in the proof are generated in such a way that
if a certain disk is put into a clique then all copies of that disk are put into the
same clique, and (ii) the maximum size of a clique in $F$ is~4, since the intersection graph of $F$ is planar.
These two facts together imply that any clique in~$\C_i$ consists of all copies
of up to four disks~$D_v$. Thus, if we define $\sep$ to contain all nodes~$v\in V$
such that the copies of~$D_v$ are in $\D_{\bd}(H_i)\cup \D_{\mylarge}$, then we obtain
a separator~$\sep$ that is balanced with respect to the costs of the nodes and such that
$\sum_{v\in \sep} \log \weight(v) = O(\sqrt{W})$.
\mdb{Hmm, maybe all of this should be explained a but better.}
\end{proof}
%--------------------------------------------------------------------------------------
